Learning Policies for Continuous Control via Transition Models

It is doubtful that animals have perfect inverse models of their limbs (e.g., what muscle contraction must be applied to every joint to reach a particular location in space). However, in robot control, moving an arm's end-effector to a target position or along a target trajectory requires accurate forward and inverse models. Here we show that by learning the transition (forward) model from interaction, we can use it to drive the learning of an amortized policy. Hence, we revisit policy optimization in relation to the deep active inference framework and describe a modular neural network architecture that simultaneously learns the system dynamics from prediction errors and the stochastic policy that generates suitable continuous control commands to reach a desired reference position. We evaluated the model by comparing it against the baseline of a linear quadratic regulator, and conclude with additional steps to take toward human-like motor control.

==> summary.tex <==
\section*{Motor Learning and Control in Humans}

\paragraph{Motor Learning} \cite{Krakauer2019}:

In this extensive review, the authors describe a wide range of phenomena related to motor learning and movement execution, spanning several scales of time from sequence learning, action selection, motor planning, action execution and adaptation in both discrete and continuous domains. They summarize from a large body of behavioral and neural data that there are different levels of cognitive systems involved in many of these processes and relate these findings to several theories dominant in the field. Interestingly enough, active inference is not mentioned a single time in the 52 pages, but instead they do speak about prediction error driven learning with forward and inverse models (especially regarding the cerebellum). They also mention the role of reward (and the difference to loss) in motor learning and can conclude that it plays in a role in some, but not all learning processes (such as adaptation). They describe nicely the findings of several reaching experiments where participants have to adapt to perturbations and their washout.

\section*{Active Inference Theory}

\paragraph{What is Optimal about Motor Control?} \cite{Friston2011}:

Friston aims to answer the question weather optimal control theory is helpful or hindering in the attempt to explain motor behavior. In an attempt to answer the question he promotes investigation of these processes under the regime of Bayesian inference. He shows the differences between three different points of view: 1) optimal control utilizes forward models for state prediction and (separately) cost functions for action selection. 2) Predictive coding where the perception is partially driven by own predictions about the world with top down predictions and bottom up predictions errors flowing primarily along the perception hierarchy. 3) Active inference where actions are, similarly to perception, driven directly by proprioceptive prediction errors and cost functions are replaced by prior believes about the world including what constitutes good states (?). He thereby extends the inference paradigm to actions (hence the name) and states that AIF can be understood as predictive coding with motor reflexes. An optimal trajectory is then just obtained from the movement with the greatest posterior probability given the current context of the agent. 

\paragraph{Predictions not commands: active inference in the motor system} \cite{Adams2013}:

In this paper, Friston et al. double down on the idea of active inference, in which higher cortical levels send descending proprioceptive predictions, rather than motor commands. They describe this process strongly related to the ideas of perceptual inference in sensory cortex, where according to the predictive coding paradigm, descending connections convey predictions, while ascending connections convey prediction errors. They aim to replace the notion of forward and inverse models with a hierarchical generative model of sensory perception and motor areas. They start out by once again comparing AIF to optimal motor control from a theoretic point of view, but this time give specific potential implementation circuitry of different neurons and brain areas to support their claims. According to the data they present (reviewed from many other studies), the somatomotor and somatosensory systems are very alike, which is in line with AIF, but not with the view that the brain performs something alike optimal control. 

\paragraph{Active Inference in Robotics and Artificial Agents: Survey and Challenges} \cite{Lanillos2021}:

The authors summarize the mathematical framework of AIF with respect to perception, control, planning, and learning and review recent advancements in these domains across literature, with a focus on robotic applications. They further summarize the relationship between control theory and RL. In summary, the authors provide an important reference for people working in this domain of research. Relevant to my research is the derivation of the Laplace approximation in the appendix.

\section*{Active Inference Implementations}

\paragraph{Active inference and robot control:a case study} \cite{piolopez2016}:

In this paper, the authors implement AIF in to control a robot arm in simulation. They do so by deriving the generative forward model from the kinematic equations of motion, so no learning or neural network models are really involved, just pure math. They demonstrate that in this abstract setting, state prediction errors can drive movement through a hierarchical model when some preferred global prior is assumed. The system is somewhat robust to noise and future iterations may serve as a basis for a model of Parkinson's disease. Friston goes on to describe how in AIF all the heavy lifting is done by the generative model which needs preferred (attractor) states that can be simple fixed-points (e.g. target reaching) or trajectories (e.g. walking).

\section*{Deep Active Inference Implementations}

\paragraph{Deep active inference} \cite{Ueltzhoeffer2018}:

The author describes how the FEP in its functional form is based on the minimization of the variational upper bound on an agent's surprise by utilizing probabilistic generative models of the world. This is the first paper to propose that these models can be approximated deep and recurrent neural networks to learn the world's dynamics and the in turn use these models in perception, planning, and action infernce (dAIF). The author goes on to derive the mathematical formalization of free energy from entropy and then minimizes the derived ELBO loss in the mountain car control task. The recurrent generative model successfully learns the dynamics and continuous control for this environment, including its own representation of velocity. The author computes continuous actions in a manner that required them to know the partial derivatives of the sensations given the action, which means propagating through the environmental dynamics, which are unknown. Therefore, this implementation uses evolutionary strategies to explore the parameters space of the generative model.

\paragraph{Bayesian Policy Selection using Active Inference} \cite{Catal2019}:

The authors implement a dAIF agent to solbe the mountain car problem from partially observable state (no velocity). They learn a probabilistic predictive perception model and use this for planning by performing rollouts of imagined action trajectories and choosing the initial action that minimized the distance to the preferred prior trajectory. That prior can either be learned via rewards (RL) or from an expert demonstration. All in all this paper is extremely similar to the one they publish a year later. There is again no comparison to any baseline or such. It is just (once again) claimed that dAIF is much cooler than dRL because the prior is more flexible and surprise minimization resembles curiosity. 

\paragraph{Learning Perception and Planning with Deep Active Inference} \cite{Catal2020}:

The authors implement a dAIF agent to solve the mountain car problem from fully observable state with only two discrete actions. They learn a probabilistic, predictive perception model and use this for planning by Monte Carlo sampling for future trajectories of a given length. In their loss function they balance surprise minimization (exploration) with visiting preferred states via a hand tuned hyper-parameter. How the preferred state (called global prior) is given is never mentioned and reward is also completely absent from the equations shown. There is no comparison to any baseline model whatsoever.

\paragraph{Deep active inference as variational policy gradients} \cite{Millidge2020}:

In order to scale the applicability of AIF, the author uses deep neural networks to approximate key densities in the AIF framework. He compares the his approach to maximum-entropy reinforcement learning and the policy gradients algorithm in theory as well as performance and concludes that they have many similarities. His implementation is end-to-end differentiable, the loss function includes the same reward maximization as known from standard RL, and these models solve three fully observable control tasks (cartpole et al). In the discussion he proposes to extend the implementation to a predictive coding network after Whittington and Bogacz to be closer to a biologically plausible process. Somehow, he claims to have scaled dAIF to "large-scale" tasks, but since he also operates directly on the fairly low dimensional, fully observable state of the continuous control environments, I am not sure this is very fitting. Also his plots are crap.

\paragraph{Deep Active inference for Partially Observable MDPs} \cite{vanderHimst2020}:

The authors present an implementation of dAIF to control the cartpole task with discrete actions while observing only pixel input (partially observable). All relevant densities to compute the variational free energy are approximated by deep neural networks. The image input is encoded into a low-dimensional latent representation via a VAE. The surprise minimization of the traditional FEP equations has been replaced with reward maximization, effectively turning the implementation into one of entropy-based dRL. The model successfully outperforms DQN on the PO control tasks, and is about the same in the fully observable case.

\section*{Deep Reinforcement Learning Implementations}

\paragraph{Mastering Atari with Discrete World Models} \cite{Hafner2020}:

The authors introduce DreamerV2, a reinforcement learning agent that learns behaviors purely from predictions in the compact latent space of a powerful world model. Image inputs of discrete input Atari games are encoded into a discrete latent representation. The generative world model is used for imagining during learning and as such DreamerV2 is related to model based RL, although it does not use the model for planning as done by MuZero. With this method, they set a new state of the art in RL for Atari games while being trained on a single GPU. The loss function includes an entropy term to facilitate exploration, which is related to AIF, as this term naturally occurs from the free energy minimization. 

\paragraph{Stochastic Latent Actor-Critic: Deep Reinforcement Learning with a Latent Variable Model} \cite{Lee2020}:

The authors aim to use existing entropy based dRL methods, specifically SAC, and extend this by a learned latent model to handle POMDPs. However, as representation learning is hard, they jointly learn the encoding via a VAE as well as the latent dynamics and hence call their implementation SLAC. However, they only use the latent state representation for the critic model (value estimation), but not for the policy, which still receives raw pixel input. They argue that a latent-conditioned actor could lead to overconfident behaviors in uncertain environments. However, this leads to the algorithm not using any imagination or planning, in contrast to e.g. DreamerV2, and can hence be considered as model free. The loss once again includes an entropy term with some weight parameter, making this model related to other variational inference models of dAIF. They evaluate their algorithm against other dRL methods on continuous control tasks of the DeepMind Control Suite and achieve state-of-the-art results. 

\section*{Alternative Approaches to Robot Control}

\paragraph{A spiking neural model of adaptive arm control} \cite{DeWolf2016}:

The authors develop a fully spiking model of the motor pathways (cortex areas and cerebellum). They use this model to control a three link robotic arm that can adapt to changes in the movement dynamics. This model is fully engineered including the kinematic equations directly into the model. The only learning occurring is the online adaptation to perturbations in the cerebellum model. They perform the reaching task and compare to human data to find that performance and spiking activity is strikingly similar to humans and primates respectively. 

\paragraph{A Bio-inspired Spiking Neural Network for Control of A 4-DoF Robotic Arm} \cite{Chen2020}:

The authors use a SNN to learn the inverse model of a robot arm. Specifically, there is a single weight matrix in a small network that is updated via supervised learning (tempotron learning rule). Joint positions are encoded in a discretized fashion and then transformed into a sparse temporal code. However, their results are not great and the arm cannot always reach the target position. 

\paragraph{Dynamic Action Inference with Recurrent Spiking Neural Networks} \cite{Traub2021}:

In this paper, the authors use a LSNN consisting of LIF and ALIF neurons to learn a model of its control dynamics as well as the world around the agent. They train the predictive model via online learning (effectively batch size = 1) with e-prop and achieve comparable results to the BPTT baseline. The predictive model is then used via MPC to unroll state trajectories, where behaviour (target seeking and obstacle avoidance) is achieved by using BPTT to get the gradient with respect to the action of a given cost function. Why they are so proud of the fact that they use biologically plausible e-prop to learn the model, only to then use a very implausible control regime based on BPTT and temporarily stored hidden network states I am not quite sure. The method works well for medium range planning trajectories, but fails when these get too long. 

\section*{Alternative Flavors of Inference}

\paragraph{Hybrid Predictive Coding: Inferring, Fast and Slow} \cite{Tschantz2022}:

The authors develop a new framework of predictive processing, which combines the classic, top-down iterative inference of predictive coding with bottom-up amortized inference to jointly optimize a single unified energy function using only local Hebbian updates. Here, both predictions as well as prediction errors are flowing both directions along the hierarchical neural model, learning both a generative model and discriminative components. They show in a proof-of-concept study that this hybrid model can learn to classify as well as generate MNIST images after having only been provided few data, and is inherently able to detect its own uncertainty and adaptively respond to changes in the environments. Hybrid predictive coding offers a new perspective on the biological relevance of the feedforward sweeps and iterative recurrent activity observed in the visual cortex during perceptual tasks.

\paragraph{Control as Hybrid Inference} \cite{Tschantz2020}:

The authors combine model-based with model-free RL control by using simultaneously iterative as well as amortized inference to obtain control signals. They verify their method on a continuous control task (half cheetah) and show that their method can utilize the sample efficiency of model-based planning while retaining the asymptotic performance of model-free policy optimisation. The CHI framework provides a hypothesis that model-free and model-based mechanisms coexist and compete in the brain according to their relative uncertainty, as well as explaining habituation as the gradual transition from goal-directed to habitual action after sufficient experience. In contrast to their later work on hybrid predictive coding, however, the implementation is not in a biologically plausible message passing regime, which would be a super interesting next move if you ask me.

\pagebreak
